Learning Causal Bayesian Networks from Text

Causal relationships form the basis for reasoning and decision-making in Artificial Intelligence systems. To exploit the large volume of textual data available today, the automatic discovery of causal relationships from text has emerged as a significant challenge in recent years. Existing approaches in this realm are limited to the extraction of low-level relations among individual events. To overcome the limitations of the existing approaches, in this paper, we propose a method for automatic inference of causal relationships from human written language at conceptual level. To this end, we leverage the characteristics of hierarchy of concepts and linguistic variables created from text, and represent the extracted causal relationships in the form of a Causal Bayesian Network. Our experiments demonstrate superiority of our approach over the existing approaches in inferring complex causal reasoning from the text.

==> 3-background.tex <==
Bayesian Network (BN), also know as belief network, is a type of Probabilistic Graphical Model (PGM) for representing multivariate probability distribution. Each node in a BN represents a variable, with a corresponding value, and each link shows the dependence between variables. In a Causal BN, the links represent causal dependency rather than the dependence.


To create a Causal Bayesian Network from textual data, let $G$ be our graphical model, and $V=\{V_1, V_2,...,V_n\}$ be the set of extracted linguistic variables (as defined in \ref{ling}) from our corpus $\zeta$. We define $Pa_{V_i}^{G} = \{Vj: Vj \xrightarrow{causal} V_i \}$, indicating set of nodes in $\zeta$ which have causal relation with $V_i$. By expressing $P$ as:
\begin{equation}
P(V_{1}, V_{2}, ..., V_{n}) = \prod_{i=1}^{n}P(V_i|Pa_{V_i}^{G})
\end{equation}
we can argue that $P$ factorises over $G$. The individual factor $P(V_i|Pa_{V_i}^{G})$ is called conditional probability distribution (explained in \ref{cpd}). In a more formal way, we define Causal Bayesian Network over our corpus $\zeta$ as $\beta =(G,P)$ where $P$ is set of conditional probability distributions.


%Using the causal relations and probabilities, conducting bayesian inference is possible with a Causal Bayesian Network(CBN). A simple version of inference using a CBN is to calculate the joint probability of a variable for a specific assignment of values for each variable in a network. A more complicated form of inference is to find the probability of a subset of variables ($V^1$), given assignment of other variables ($e$):
%\begin{equation}  
%P(V^1|e) = \alpha \sum_{\forall V^2 \in V} P(V^1,e,V^2)
%\end{equation}
%where $V^2$ denotes set of variables that don't exist in $V^1$ and \textit{e}, and $\alpha$ is a normalisation constant.


In addition to the aforementioned usages of a CBN, having a Causal Bayesian Networks enables the possibility of answering questions in three different layers \cite{pearl2018book}: The Association layer answers statistical relation based on observation between the two variables $P(V_i|V_j)$; the Intervention layer answers to the act of changing in the observation $P(V_i|do(V_j))$; and the Counter-factual layer answers to the imaginary question, which is based on an alternation in a previous situation $P(V_{i_{V_j}} | V_i^{'}, V_j^{'})$. 
While most of current AI systems works on only the first layer, the outcome of this paper empowers current AI to climb up to the next layers and perform a better reasoning and decision making by filling this gap.
